Automatic Recognition of Landmarks on Digital Dental Models

Fundamental to improving Dental and Orthodontic treatments is the ability to quantitatively assess and cross-compare their outcomes. Such assessments require calculating distances and angles from 3D coordinates of dental landmarks. The costly and repetitive task of hand-labelling dental models impedes studies requiring large sample size to penetrate statistical noise. We have developed techniques and software implementing these techniques to map out automatically, 3D dental scans. This process is divided into consecutive steps - determining a model's orientation, separating and identifying the individual tooth and finding landmarks on each tooth - described in this paper. Examples to demonstrate techniques and the software and discussions on remaining issues are provided as well. The software is originally designed to automate Modified Huddard Bodemham (MHB) landmarking for assessing cleft lip/palate patients. Currently only MHB landmarks are supported, but is extendable to any predetermined landmarks. This software, coupled with intra-oral scanning innovation, should supersede the arduous and error prone plaster model and caliper approach to Dental research and provide a stepping-stone towards automation of routine clinical assessments such as "index of orthodontic treatment need" (IOTN).

==> results/old-results.tex <==
\section{Results}

Multiple experiments were done to assess the software's performance. These are split into a qualitative \emph{did it find the right tooth?} test, a quantitative \emph{how precise were the landmarks placed?}, and quantitative consistency test.


\subsection{Qualitative Reliability}

A qualitative assessment of the software's ability to identify teeth was performed on all the models listed in table~\ref{tab:models-counts}. Teeth were labelled by hand and by the machine and compared on a per-tooth basis. Tables \ref{tab:qualititive-counts} and \ref{tab:qualititive-ratios} provide summary statistics as raw counts and as percentages respectively. 

\begin{table}[!ht]
\centering
\begin{tabular}{lccc}
\toprule
{}               &  Cast  &  IO    &  Cast      \\
{}               &  Adult &  Adult &  Deciduous \\
\midrule
OK               &    475 &    157 &        894 \\
Partition Error  &     46 &     28 &        136 \\
Wrong Assignment &     67 &     25 &         87 \\
Wrong kind       &     22 &      9 &         32 \\
\bottomrule
\end{tabular}
\caption{Per-tooth qualitative \emph{did it find the correct tooth?} counts.}
\label{tab:qualititive-counts}
\end{table}

\begin{table}[!ht]
\centering
\begin{tabular}{lccc}
\toprule
{}               &  Cast  &  IO    &  Cast      \\
{}               &  Adult &  Adult &  Deciduous \\
\midrule
OK               &       80.8\% &     74.8\% &           80.0\% \\
Partition Error  &        7.8\% &     13.3\% &           12.2\% \\
Wrong Assignment &       11.4\% &     11.9\% &            7.8\% \\
Wrong kind       &        3.7\% &      4.3\% &            2.9\% \\
\bottomrule
\end{tabular}
\caption{The counts from table~\ref{tab:qualititive-counts} as percentages of all teeth in that group of models.}
\label{tab:qualititive-ratios}
\end{table}

\paragraph{Table Key:}

\begin{itemize}[noitemsep]
    \item \emph{OK} : the software found and labelled the tooth correctly.
    \item \emph{Partition Error} : the tooth was not found in section~\ref{sec:partition-into-individual-teeth}.
    \item \emph{Wrong Assignment} : the tooth was found but mislabelled in section~\ref{sec:tooth-assignment} (most of which where lower incisors).
    \item \emph{Wrong kind}, a subset of \emph{Wrong Assignment}, is where the software also chose incorrectly from incisor, canine, premolar and molar.
\end{itemize}

In addition to the mistakes above, one deciduous model failed at the orientation stage. The \textit{find peaks points} stage had no issues.

These qualitative mistakes are by far the area in which the software needs the most development. With its current rates of reliability, landmarks generated will almost certainly need to be proof-checked and amended by a human examiner placing or relabelling the missing or mislabeled landmarks. 


\subsection{Quantitative Accuracy}

\emph{Of the teeth that are correctly found and labelled by the software, how accurate are the landmarks placed on the teeth?}

The accuracy of the landmarks placed is somewhat ambiguous to measure as it requires knowing true positions of the landmarks - which are subjective. But our approach to approximate it is as follows:

Three human examiners, with sufficient expertise, and the software each independently placed MHB landmarks on 20 dental models (10 upper/lower pairs). Any teeth which the software failed to identify correctly were excluded. A \textit{consensus landmark} for each tooth was obtained by taking a mean of the landmarks from each examiner (including the software). An overall \textit{discrepancy score} for each examiner was obtained by calculating the mean distance between each examiner's landmarks and the \textit{consensus landmark}. We consider the software to be as accurate as the humans if its discrepancy score is no higher than the humans' scores.

\begin{table}[!ht]
    \centering
    \begin{tabular}{lcccc}
    \hline
     Deviation    &  {}  &   \multicolumn{3}{c}{Humans} \\
    (mm) & Software & A & B & C \\
\hline
 Incisors         &      0.454 &     0.565 &     0.387 &     0.349 \\
 Canines          &      0.369 &     0.630 &     0.322 &     0.291 \\
 Premolars        &      0.402 &     0.472 &     0.313 &     0.296 \\
 Molars           &      0.334 &     0.382 &     0.269 &     0.310 \\
 Overall          &      0.389 &     0.517 &     0.310 &     0.300 \\
\hline
    \end{tabular}
    \caption{Landmark Deviation Errors}
    \label{tab:accuracy}
\end{table}

It's also worth pointing out that for four models, a human examiner confused left with right, which had to be corrected before any of the above calculations. This is a classic human mistake that the software will never make.

\subsection{Repeatability}

Self-consistency doesn't necessarily imply accuracy but self-inconsistency would certainly tell us that the results from this software are untrustworthy. We therefore test for self-inconsistency to assure ourselves that this is not the case.

The usual methods to evaluate self-consistency (or inter-rater reliability) in humans - just repeat the experiment again the next week and compare results - don't apply to software. No matter how poor a software is, it will always yield exactly the same output for the same input, giving a misleading perfect self-consistency in all tests. To get around this we need an equivalent, but not identical input. To do this we:

\begin{itemize}[noitemsep]
    \item Re-scan a sub-sample  of 14 of our plaster models.
    \item Use the software to find landmarks on both scans.
    \item Find a transform that will map the original model onto the re-scanned one using techniques from AutoIDD~\cite{REESU2020110218}. (AutoIDD doesn't use the landmarks - this step is independent of the previous one.)
    \item Apply the transform to the landmarks of the original model and compare to the landmarks of the re-scanned model.
\end{itemize}

The results are a mean and median distance of $0.212mm$ and $0.160mm$ respectively. This, being substantially lower than the deviation between human examiners in table~\ref{tab:accuracy}, is highly encouraging. The mean being higher than the median correctly implies that there are a few high outliers (usually worn cusp tips) dragging the mean up. Note, the scanner's accuracy has been estimated (again using AutoIDD) to be around $0.06mm$. This implies a noise floor and an ideal target value (which we're not hitting) for our landmark software of around that value.



